Nonlinear Trajectory Optimization Models for Uncrewed Aerial Vehicles with Mobile Charging Support

Supporting Uncrewed Aerial Vehicles (UAVs) with mobile charging stations enables persistent UAV autonomy in infrastructure-sparse environments. In this setting, trajectory optimization for UAVs is challenging because it couples task scheduling with when and where to recharge, as well as terrain-access constraints on where charging is available. We propose a smooth nonlinear trajectory optimization model for UAV with mobile charging support. Compared with existing results, the proposed model allows nonlinear charging dynamics mode via a unified battery dynamics model with disjunctive constraints on the time allocated to each mode. Furthermore, it provides smooth approximations of the disjunctive constraints with bounded approximation errors. By avoiding integer variables, these approximations enable efficient solution using smooth nonlinear optimization algorithms. We evaluate the proposed model on UAV missions with multiple spatially distributed tasks, nonlinear constant-current--constant-voltage charging dynamics, and terrain-access constraints on mobile charging support. Compared with mixed-integer nonlinear programs, the proposed model provides high-quality approximate solutions while reducing the computation time by orders of magnitude.

==> MINLP_10/boxplot_body_10.tex <==
% Paired NLP / MINLP (Juniper) comparison.
% Centers: NLP at j-0.20; Juniper at j+0.20.
% Box width 0.26; dots span +/-0.11 around their own center.
\providecommand{\NLPBoxColor}{red}
\providecommand{\NLPSampleOpacity}{0.45}
\pgfplotstableread[col sep=tab]{\BoxFile}\PreparedBoxes
\pgfplotstableread[col sep=tab]{\NLPBoxFile}\PreparedNLPBoxes
\providecolor{MINLP_color}{rgb}{0,0.447,0.741}

\begin{tikzpicture}[trim axis left, trim axis right]
\begin{axis}[
    xlabel={\PlotXLabel},
    ylabel={\PlotYLabel},
    ymode=\PlotYMode,
    label style={font=\footnotesize},
    tick label style={font=\scriptsize},
    width=1.0\linewidth,
    height=0.45\linewidth,
    xmin=0.5,
    xmax=9.5,
    xtick={1,2,3,4,5,6,7,8,9},
    boxplot/draw direction=y,
    unbounded coords=discard,
]

% Keep the existing Juniper legend name so the main figure still works.
\ifdefined\MakeSharedLegend
    \pgfplotsset{
        legend to name=minlp_sharedlegend_MINLP_10,
        legend columns=-1,
        legend style={draw=none, font=\footnotesize,
        /tikz/every even column/.append style={column sep = 6pt}}
    }
    \addlegendimage{area legend, draw=red,
        fill=red!20, line width=0.6pt}
    \addlegendentry{NLP}
    \addlegendimage{area legend, draw=MINLP_color,
        fill=MINLP_color!20, line width=0.6pt}
    \addlegendentry{MINLP (Juniper, 10 h)}
\fi

% All original samples; jitter stays inside each series' column.
\pgfmathsetseed{123}
\pgfplotsinvokeforeach{1,...,9}{
    \addplot[forget plot, only marks, mark=*, mark size=0.35pt,
        color=red, opacity=\NLPSampleOpacity]
    table[col sep=tab, x expr={#1-0.20+0.22*(rnd-0.5)},
        y=aoi#1]{\NLPSampleFile};
}
\pgfmathsetseed{123}
\pgfplotsinvokeforeach{1,...,9}{
    \addplot[forget plot, only marks, mark=*, mark size=0.35pt,
        color=MINLP_color, opacity=0.45]
    table[col sep=tab, x expr={#1+0.20+0.22*(rnd-0.5)},
        y=aoi#1]{\SampleFile};
}


% Red NLP boxes (left).
% Prepared boxes: nine data rows, indexed from 0 to 8.
\pgfplotsinvokeforeach{0,...,8}{
    \pgfplotstablegetelem{#1}{aois}\of\PreparedNLPBoxes
    \edef\AOI{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerWhisker}\of\PreparedNLPBoxes
    \edef\LW{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerQuartile}\of\PreparedNLPBoxes
    \edef\LQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{median}\of\PreparedNLPBoxes
    \edef\MED{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperQuartile}\of\PreparedNLPBoxes
    \edef\UQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperWhisker}\of\PreparedNLPBoxes
    \edef\UW{\pgfplotsretval}

    \edef\DrawBox{
        \noexpand\addplot+[
            forget plot,
            boxplot prepared={
                draw position={\AOI-0.20},
                lower whisker=\LW,
                lower quartile=\LQ,
                median=\MED,
                upper quartile=\UQ,
                upper whisker=\UW
            },
            boxplot/box extend=0.26,
            boxplot/every whisker/.style={draw=none},
            draw=red,
            fill=red!20,
            line width=0.6pt,
            fill opacity=0.2,
            draw opacity=1,
            draw=\NLPBoxColor,
            mark=none
        ] coordinates {};
    }
    \DrawBox
}

% Blue Juniper boxes (right).
% Prepared boxes: nine data rows, indexed from 0 to 8.
\pgfplotsinvokeforeach{0,...,8}{
    \pgfplotstablegetelem{#1}{Count}\of\PreparedBoxes
    \ifnum\pgfplotsretval>0\relax
    \pgfplotstablegetelem{#1}{aois}\of\PreparedBoxes
    \edef\AOI{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerWhisker}\of\PreparedBoxes
    \edef\LW{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerQuartile}\of\PreparedBoxes
    \edef\LQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{median}\of\PreparedBoxes
    \edef\MED{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperQuartile}\of\PreparedBoxes
    \edef\UQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperWhisker}\of\PreparedBoxes
    \edef\UW{\pgfplotsretval}

    \edef\DrawBox{
        \noexpand\addplot+[
            forget plot,
            boxplot prepared={
                draw position={\AOI+0.20},
                lower whisker=\LW,
                lower quartile=\LQ,
                median=\MED,
                upper quartile=\UQ,
                upper whisker=\UW
            },
            boxplot/box extend=0.26,
            boxplot/every whisker/.style={draw=none},
            draw=MINLP_color,
            fill=MINLP_color!20,
            line width=0.6pt,
            fill opacity=0.2,
            draw opacity=1,
            mark=none
        ] coordinates {};
    }
    \DrawBox
    \fi
}



\end{axis}
\end{tikzpicture}


==> MINLP_10/obj_plot_10.tex <==
\begingroup
\def\PlotXLabel{}
\def\MakeSharedLegend{1}
\def\PlotYMode{normal}
\def\BoxFile{MINLP_10/MINLP_obj_boxes.dat}
\def\SampleFile{MINLP_10/MINLP_obj_samples.dat}
\def\PlotYLabel{Objective (h)}

\def\NLPBoxFile{NLP_plot/NLP_obj_boxes.dat}
\def\NLPSampleFile{NLP_plot/NLP_obj_samples.dat}
\input{MINLP_10/boxplot_body_10.tex}
\endgroup


==> MINLP_10/time_plot_10.tex <==
\begingroup
\def\PlotYMode{log}
\def\BoxFile{MINLP_10/MINLP_time_boxes.dat}
\def\SampleFile{MINLP_10/MINLP_time_samples.dat}
\def\PlotYLabel{Computation time (min)}
\def\PlotXLabel{}
\def\NLPBoxFile{NLP_plot/NLP_time_boxes.dat}
\def\NLPSampleFile{NLP_plot/NLP_time_samples.dat}
\pgfplotsset{every axis/.append style={
    ytick={0.1,1,10,100,1000},
    minor ytick={
        0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,
        2,3,4,5,6,7,8,9,
        20,30,40,50,60,70,80,90,
        200,300,400,500,600,700,800,900
    },
    minor tick length=2pt,
    execute at end axis={
        \addplot[
            gray,
            dashed,
            thin,
            no marks,
            forget plot
        ] coordinates {
            (\pgfkeysvalueof{/pgfplots/xmin},600)
            (\pgfkeysvalueof{/pgfplots/xmax},600)
        };
    }
}}

\input{MINLP_10/boxplot_body_10.tex}
\endgroup


==> MINLP_10/vio_plot_10.tex <==
\begingroup
\def\PlotXLabel{Number of UAV task locations \(m^{\mathrm{A}}\)}
\def\PlotYMode{log}
\def\BoxFile{MINLP_10/MINLP_vio_boxes.dat}
\def\SampleFile{MINLP_10/MINLP_vio_samples.dat}
\def\PlotYLabel{Constraint violation}
\def\NLPBoxFile{NLP_plot/NLP_vio_boxes.dat}
\def\NLPSampleFile{NLP_plot/NLP_vio_samples.dat}


\pgfplotsset{every axis/.append style={
    ytick={1e-11,1e-7,1e-3},
    minor ytick={1e-10, 1e-9,1e-8,1e-6,1e-5,1e-4},
    minor tick length=2pt
}}


\input{MINLP_10/boxplot_body_10.tex}
\endgroup


==> MINLP_SCIP/boxplot_body_SCIP.tex <==
% Three methods: NLP (left), SCIP (middle), Juniper (right).
% Centers: NLP at j-0.28; SCIP at j; Juniper at j+0.28.
% Box width 0.20; sample jitter spans +/-0.08.
\providecommand{\NLPBoxColor}{red}
\providecommand{\NLPSampleOpacity}{0.45}
\pgfplotstableread[col sep=tab]{\BoxFile}\PreparedBoxes
\pgfplotstableread[col sep=tab]{\NLPBoxFile}\PreparedNLPBoxes
\pgfplotstableread[col sep=tab]{\JuniperBoxFile}\PreparedJuniperBoxes
\definecolor{Juniper_color}{rgb}{0,0.50,0.30}
\providecolor{MINLP_color}{rgb}{0,0.447,0.741}

\begin{tikzpicture}[trim axis left, trim axis right]
\begin{axis}[
    xlabel={\PlotXLabel},
    ylabel={\PlotYLabel},
    ymode=\PlotYMode,
    label style={font=\footnotesize},
    tick label style={font=\scriptsize},
    width=0.9\linewidth,
    height=0.45\linewidth,
    xmin=0.5,
    xmax=9.5,
    xtick={1,2,3,4,5,6,7,8,9},
    boxplot/draw direction=y,
    unbounded coords=discard,
]

% Keep the existing SCIP legend name so the main figure still works.
\ifdefined\MakeSharedLegend
    \pgfplotsset{
        legend to name=three_methods_sharedlegend,
        legend columns=-1,
        legend style={draw=none, font=\scriptsize,
        /tikz/every even column/.append style={column sep = 6pt}}
    }
    \addlegendimage{area legend, draw=red,
        fill=red!20, line width=0.6pt}
    \addlegendentry{NLP}
    \addlegendimage{area legend, draw=MINLP_color,
        fill=MINLP_color!20, line width=0.6pt}
    \addlegendentry{MINLP (SCIP)}
    \addlegendimage{area legend, draw=Juniper_color,
        fill=Juniper_color!20, line width=0.6pt}
    \addlegendentry{MINLP (Juniper)}
\fi

% All original samples; jitter stays inside each series' column.
\pgfmathsetseed{123}
\pgfplotsinvokeforeach{1,...,9}{
    \addplot[forget plot, only marks, mark=*, mark size=0.35pt,
        color=red, opacity=\NLPSampleOpacity]
    table[col sep=tab, x expr={#1-0.28+0.16*(rnd-0.5)},
        y=aoi#1]{\NLPSampleFile};
}
\pgfmathsetseed{123}
\pgfplotsinvokeforeach{1,...,9}{
    \addplot[forget plot, only marks, mark=*, mark size=0.35pt,
        color=MINLP_color, opacity=0.45]
    table[col sep=tab, x expr={#1+0.16*(rnd-0.5)},
        y=aoi#1]{\SampleFile};
}


\pgfmathsetseed{123}
\pgfplotsinvokeforeach{1,...,9}{
    \addplot[forget plot, only marks, mark=*, mark size=0.35pt,
        color=Juniper_color, opacity=0.45]
    table[col sep=tab, x expr={#1+0.28+0.16*(rnd-0.5)},
        y=aoi#1]{\JuniperSampleFile};
}


% Red NLP boxes (left).
% Prepared boxes: nine data rows, indexed from 0 to 8.
\pgfplotsinvokeforeach{0,...,8}{
    \pgfplotstablegetelem{#1}{aois}\of\PreparedNLPBoxes
    \edef\AOI{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerWhisker}\of\PreparedNLPBoxes
    \edef\LW{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerQuartile}\of\PreparedNLPBoxes
    \edef\LQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{median}\of\PreparedNLPBoxes
    \edef\MED{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperQuartile}\of\PreparedNLPBoxes
    \edef\UQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperWhisker}\of\PreparedNLPBoxes
    \edef\UW{\pgfplotsretval}

    \edef\DrawBox{
        \noexpand\addplot+[
            forget plot,
            boxplot prepared={
                draw position={\AOI-0.28},
                lower whisker=\LW,
                lower quartile=\LQ,
                median=\MED,
                upper quartile=\UQ,
                upper whisker=\UW
            },
            boxplot/box extend=0.20,
            boxplot/every whisker/.style={draw=none},
            draw=red,
            fill=red!20,
            line width=0.6pt,
            fill opacity=0.2,
            draw opacity=1,
            draw=\NLPBoxColor,
            mark=none
        ] coordinates {};
    }
    \DrawBox
}

% Blue SCIP boxes (middle).
% Prepared boxes: nine data rows, indexed from 0 to 8.
\pgfplotsinvokeforeach{0,...,8}{
    \pgfplotstablegetelem{#1}{Count}\of\PreparedBoxes
    \ifnum\pgfplotsretval>0\relax
    \pgfplotstablegetelem{#1}{aois}\of\PreparedBoxes
    \edef\AOI{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerWhisker}\of\PreparedBoxes
    \edef\LW{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerQuartile}\of\PreparedBoxes
    \edef\LQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{median}\of\PreparedBoxes
    \edef\MED{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperQuartile}\of\PreparedBoxes
    \edef\UQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperWhisker}\of\PreparedBoxes
    \edef\UW{\pgfplotsretval}

    \edef\DrawBox{
        \noexpand\addplot+[
            forget plot,
            boxplot prepared={
                draw position={\AOI},
                lower whisker=\LW,
                lower quartile=\LQ,
                median=\MED,
                upper quartile=\UQ,
                upper whisker=\UW
            },
            boxplot/box extend=0.20,
            boxplot/every whisker/.style={draw=none},
            draw=MINLP_color,
            fill=MINLP_color!20,
            line width=0.6pt,
            fill opacity=0.2,
            draw opacity=1,
            mark=none
        ] coordinates {};
    }
    \DrawBox
    \fi
}



% Green Juniper boxes (right).
% Prepared boxes: nine data rows, indexed from 0 to 8.
\pgfplotsinvokeforeach{0,...,8}{
    \pgfplotstablegetelem{#1}{Count}\of\PreparedJuniperBoxes
    \ifnum\pgfplotsretval>0\relax
    \pgfplotstablegetelem{#1}{aois}\of\PreparedJuniperBoxes
    \edef\AOI{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerWhisker}\of\PreparedJuniperBoxes
    \edef\LW{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerQuartile}\of\PreparedJuniperBoxes
    \edef\LQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{median}\of\PreparedJuniperBoxes
    \edef\MED{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperQuartile}\of\PreparedJuniperBoxes
    \edef\UQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperWhisker}\of\PreparedJuniperBoxes
    \edef\UW{\pgfplotsretval}

    \edef\DrawBox{
        \noexpand\addplot+[
            forget plot,
            boxplot prepared={
                draw position={\AOI+0.28},
                lower whisker=\LW,
                lower quartile=\LQ,
                median=\MED,
                upper quartile=\UQ,
                upper whisker=\UW
            },
            boxplot/box extend=0.20,
            boxplot/every whisker/.style={draw=none},
            draw=Juniper_color,
            fill=Juniper_color!20,
            line width=0.6pt,
            fill opacity=0.2,
            draw opacity=1,
            mark=none
        ] coordinates {};
    }
    \DrawBox
    \fi
}



\end{axis}
\end{tikzpicture}


==> MINLP_SCIP/obj_plot_SCIP.tex <==
\begingroup
\def\PlotXLabel{}
\def\MakeSharedLegend{1}
\def\PlotYMode{normal}
\def\BoxFile{MINLP_SCIP/MINLP_obj_boxes.dat}
\def\SampleFile{MINLP_SCIP/MINLP_obj_samples.dat}
\def\PlotYLabel{Objective (h)}

\def\NLPBoxFile{NLP_plot/NLP_obj_boxes.dat}
\def\NLPSampleFile{NLP_plot/NLP_obj_samples.dat}
\def\JuniperBoxFile{MINLP_10/MINLP_obj_boxes.dat}
\def\JuniperSampleFile{MINLP_10/MINLP_obj_samples.dat}
\input{MINLP_SCIP/boxplot_body_SCIP.tex}
\endgroup


==> MINLP_SCIP/time_plot_SCIP.tex <==
\begingroup
\def\PlotYMode{log}
\def\BoxFile{MINLP_SCIP/MINLP_time_boxes.dat}
\def\SampleFile{MINLP_SCIP/MINLP_time_samples.dat}
\def\PlotYLabel{Computation time (min)}
\def\PlotXLabel{}
\def\NLPBoxFile{NLP_plot/NLP_time_boxes.dat}
\def\NLPSampleFile{NLP_plot/NLP_time_samples.dat}
\pgfplotsset{every axis/.append style={
    ytick={0.1,1,10,100,1000},
    minor ytick={
        0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,
        2,3,4,5,6,7,8,9,
        20,30,40,50,60,70,80,90,
        200,300,400,500,600,700,800,900
    },
    minor tick length=2pt,
    execute at end axis={
        \addplot[
            gray,
            dashed,
            thin,
            no marks,
            forget plot
        ] coordinates {
            (\pgfkeysvalueof{/pgfplots/xmin},600)
            (\pgfkeysvalueof{/pgfplots/xmax},600)
        };
    }
}}

\def\JuniperBoxFile{MINLP_10/MINLP_time_boxes.dat}
\def\JuniperSampleFile{MINLP_10/MINLP_time_samples.dat}
\input{MINLP_SCIP/boxplot_body_SCIP.tex}
\endgroup


==> MINLP_SCIP/vio_plot_SCIP.tex <==
\begingroup
\def\PlotXLabel{Number of UAV task locations \(\tau\)}
\def\PlotYMode{log}
\def\BoxFile{MINLP_SCIP/MINLP_vio_boxes.dat}
\def\SampleFile{MINLP_SCIP/MINLP_vio_samples.dat}
\def\PlotYLabel{Constraint violation}
\def\NLPBoxFile{NLP_plot/NLP_vio_boxes.dat}
\def\NLPSampleFile{NLP_plot/NLP_vio_samples.dat}


\pgfplotsset{every axis/.append style={
    ytick={1e-11,1e-7,1e-3},
    minor ytick={1e-10, 1e-9,1e-8,1e-6,1e-5,1e-4},
    minor tick length=2pt
}}


\def\JuniperBoxFile{MINLP_10/MINLP_vio_boxes.dat}
\def\JuniperSampleFile{MINLP_10/MINLP_vio_samples.dat}
\input{MINLP_SCIP/boxplot_body_SCIP.tex}
\endgroup


==> NLP_plot/boxplot_body_NLP.tex <==
\pgfplotstableread[col sep=tab]{\BoxFile}\PreparedBoxes

\begin{tikzpicture}[trim axis left, trim axis right]

\begin{axis}[
    % xlabel={\(m^{\mathrm{A}}\)},
    xlabel={\PlotXLabel},
    ylabel={\PlotYLabel},
    ymode=\PlotYMode,
    label style={font=\footnotesize},
    tick label style={font=\scriptsize},
    width=0.9\linewidth,
    height=0.45\linewidth,
    xmin=0.5,
    xmax=9.5,
    xtick={1,2,3,4,5,6,7,8,9},
    boxplot/draw direction=y,
    unbounded coords=discard,
]

% Generate the shared legend only from the objective plot.
\ifdefined\MakeSharedLegend
    \pgfplotsset{
        legend to name=obj_sharedlegend_NLP,
        legend columns=-1,
        legend style={draw=none, font=\footnotesize}
    }

    \addlegendimage{
        area legend,
        draw=NLP_color,
        fill=NLP_color!20,
        line width=0.6pt
    }
    \addlegendentry{NLP}

    % Uncomment when MINLP data and MINLP_color are added:
    % \addlegendimage{
    %     area legend,
    %     draw=MINLP_color,
    %     fill=MINLP_color!20,
    %     line width=0.6pt
    % }
    % \addlegendentry{MINLP}
\fi



% Prepared boxes: nine data rows, indexed from 0 to 8.
\pgfplotsinvokeforeach{0,...,8}{
    \pgfplotstablegetelem{#1}{aois}\of\PreparedBoxes
    \edef\AOI{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerWhisker}\of\PreparedBoxes
    \edef\LW{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerQuartile}\of\PreparedBoxes
    \edef\LQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{median}\of\PreparedBoxes
    \edef\MED{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperQuartile}\of\PreparedBoxes
    \edef\UQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperWhisker}\of\PreparedBoxes
    \edef\UW{\pgfplotsretval}

    \edef\DrawBox{
        \noexpand\addplot+[
            forget plot,
            boxplot prepared={
                draw position=\AOI,
                lower whisker=\LW,
                lower quartile=\LQ,
                median=\MED,
                upper quartile=\UQ,
                upper whisker=\UW
            },
            boxplot/box extend=0.45,
            boxplot/every whisker/.style={draw=none},
            draw=NLP_color,
            fill=NLP_color!20,
            line width=0.6pt,
            mark=none
        ] coordinates {};
    }
    \DrawBox
}

% All samples as small dots
\pgfmathsetseed{123}

\pgfplotsinvokeforeach{1,...,9}{
    \addplot[
        forget plot,
        only marks,
        mark=*,
        mark size=0.35pt,
        color=NLP_color,
        opacity=0.45
    ]
    table[
        col sep=tab,
        x expr={#1 + 0.28*(rnd-0.5)},
        y=aoi#1
    ]{\SampleFile};
}

\end{axis}
\end{tikzpicture}


==> NLP_plot/obj_plot_NLP.tex <==
% \begingroup
% \def\PlotYMode{normal}
% \def\BoxFile{all_samples_plot/NLP_obj_boxes.dat}
% \def\SampleFile{all_samples_plot/NLP_obj_samples.dat}
% \def\PlotYLabel{Objective value}
% \input{all_samples_plot/boxplot_body.tex}
% \endgroup


\begingroup
\def\PlotXLabel{}
\def\MakeSharedLegend{1}
\def\PlotYMode{normal}
\def\BoxFile{NLP_plot/NLP_obj_boxes.dat}
\def\SampleFile{NLP_plot/NLP_obj_samples.dat}
\def\PlotYLabel{Objective (h)}

\input{NLP_plot/boxplot_body_NLP}
\endgroup

==> NLP_plot/ratio_plot_NLP.tex <==
\begingroup
\def\PlotXLabel{}
\def\PlotYMode{log}
\def\BoxFile{NLP_plot/NLP_ratio_power_p_boxes.dat}
\def\SampleFile{NLP_plot/NLP_ratio_power_p_samples.dat}
\def\PlotYLabel{Ratio}
\input{NLP_plot/boxplot_body_NLP.tex}
\endgroup


==> NLP_plot/time_plot_NLP.tex <==
\begingroup
\def\PlotYMode{log}
\def\BoxFile{NLP_plot/NLP_time_boxes.dat}
\def\SampleFile{NLP_plot/NLP_time_samples.dat}
\def\PlotYLabel{Computation time (min)}
\def\PlotXLabel{}
\input{NLP_plot/boxplot_body_NLP}
\endgroup


==> NLP_plot/vio_plot_NLP.tex <==
\begingroup
\def\PlotXLabel{Number of task locations \(m^{\mathrm{A}}\)}
\def\PlotYMode{log}
\def\BoxFile{NLP_plot/NLP_vio_boxes.dat}
\def\SampleFile{NLP_plot/NLP_vio_samples.dat}
\def\PlotYLabel{Constraint violation}
% \pgfplotsset{
%     every axis/.append style={
%         extra y ticks={1e-4,1e-6},
%         extra y tick labels={$10^{-4}$,$10^{-6}$}
%     }
% }
\input{NLP_plot/boxplot_body_NLP}
\endgroup

==> all_samples_plot/boxplot_body.tex <==
\pgfplotstableread[col sep=tab]{\BoxFile}\PreparedBoxes

\begin{tikzpicture}[trim axis left, trim axis right]

\begin{axis}[
    % xlabel={\(m^{\mathrm{A}}\)},
    xlabel={\PlotXLabel},
    ylabel={\PlotYLabel},
    ymode=\PlotYMode,
    label style={font=\footnotesize},
    tick label style={font=\scriptsize},
    width=0.9\linewidth,
    height=0.45\linewidth,
    xmin=0.5,
    xmax=9.5,
    xtick={1,2,3,4,5,6,7,8,9},
    boxplot/draw direction=y,
    unbounded coords=discard,
]

% Generate the shared legend only from the objective plot.
\ifdefined\MakeSharedLegend
    \pgfplotsset{
        legend to name=obj_sharedlegend,
        legend columns=-1,
        legend style={draw=none, font=\footnotesize}
    }

    \addlegendimage{
        area legend,
        draw=NLP_color,
        fill=NLP_color!20,
        line width=0.6pt
    }
    \addlegendentry{NLP}

    % Uncomment when MINLP data and MINLP_color are added:
    % \addlegendimage{
    %     area legend,
    %     draw=MINLP_color,
    %     fill=MINLP_color!20,
    %     line width=0.6pt
    % }
    % \addlegendentry{MINLP}
\fi



% Prepared boxes: nine data rows, indexed from 0 to 8.
\pgfplotsinvokeforeach{0,...,8}{
    \pgfplotstablegetelem{#1}{aois}\of\PreparedBoxes
    \edef\AOI{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerWhisker}\of\PreparedBoxes
    \edef\LW{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{lowerQuartile}\of\PreparedBoxes
    \edef\LQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{median}\of\PreparedBoxes
    \edef\MED{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperQuartile}\of\PreparedBoxes
    \edef\UQ{\pgfplotsretval}

    \pgfplotstablegetelem{#1}{upperWhisker}\of\PreparedBoxes
    \edef\UW{\pgfplotsretval}

    \edef\DrawBox{
        \noexpand\addplot+[
            forget plot,
            boxplot prepared={
                draw position=\AOI,
                lower whisker=\LW,
                lower quartile=\LQ,
                median=\MED,
                upper quartile=\UQ,
                upper whisker=\UW
            },
            boxplot/box extend=0.45,
            boxplot/every whisker/.style={draw=none},
            draw=NLP_color,
            fill=NLP_color!20,
            line width=0.6pt,
            mark=none
        ] coordinates {};
    }
    \DrawBox
}

% All samples as small dots
\pgfmathsetseed{123}

\pgfplotsinvokeforeach{1,...,9}{
    \addplot[
        forget plot,
        only marks,
        mark=*,
        mark size=0.35pt,
        color=NLP_color,
        opacity=0.45
    ]
    table[
        col sep=tab,
        x expr={#1 + 0.28*(rnd-0.5)},
        y=aoi#1
    ]{\SampleFile};
}

\end{axis}
\end{tikzpicture}


==> all_samples_plot/obj_plot.tex <==
% \begingroup
% \def\PlotYMode{normal}
% \def\BoxFile{all_samples_plot/NLP_obj_boxes.dat}
% \def\SampleFile{all_samples_plot/NLP_obj_samples.dat}
% \def\PlotYLabel{Objective value}
% \input{all_samples_plot/boxplot_body.tex}
% \endgroup


\begingroup
\def\PlotXLabel{}
\def\MakeSharedLegend{1}
\def\PlotYMode{normal}
\def\BoxFile{all_samples_plot/NLP_obj_boxes.dat}
\def\SampleFile{all_samples_plot/NLP_obj_samples.dat}
\def\PlotYLabel{Objective (h)}

\input{all_samples_plot/boxplot_body.tex}
\endgroup

==> all_samples_plot/ratio_plot.tex <==
\begingroup
\def\PlotXLabel{}
\def\PlotYMode{log}
\def\BoxFile{all_samples_plot/NLP_ratio_power_p_boxes.dat}
\def\SampleFile{all_samples_plot/NLP_ratio_power_p_samples.dat}
\def\PlotYLabel{Ratio}
\input{all_samples_plot/boxplot_body.tex}
\endgroup


==> all_samples_plot/time_plot.tex <==
\begingroup
\def\PlotYMode{log}
\def\BoxFile{all_samples_plot/NLP_time_boxes.dat}
\def\SampleFile{all_samples_plot/NLP_time_samples.dat}
\def\PlotYLabel{Computation time (min)}
\def\PlotXLabel{}
\input{all_samples_plot/boxplot_body.tex}
\endgroup


==> all_samples_plot/vio_plot.tex <==
\begingroup
\def\PlotXLabel{Number of task locations \(m^{\mathrm{A}}\)}
\def\PlotYMode{log}
\def\BoxFile{all_samples_plot/NLP_vio_boxes.dat}
\def\SampleFile{all_samples_plot/NLP_vio_samples.dat}
\def\PlotYLabel{Constraint violation}
% \pgfplotsset{
%     every axis/.append style={
%         extra y ticks={1e-4,1e-6},
%         extra y tick labels={$10^{-4}$,$10^{-6}$}
%     }
% }
\input{all_samples_plot/boxplot_body.tex}
\endgroup

==> figure/map.tex <==
\begin{figure}[!t]
\centering
\begin{tikzpicture}

% include the EPS figure
\node[anchor=south west, inner sep=0] (img) 
    {\includegraphics[width=0.65\linewidth]{figure/first_image_09.eps}};

% define coordinate system based on image
\begin{scope}[x={(img.south east)}, y={(img.north west)}]


\node at (0.5,-0.05) {\footnotesize $ X\;(\mathrm{km})$};
\node[rotate=90] at (-0.05,0.5) {\footnotesize $ Y\;(\mathrm{km})$};

\node at (0.29,0.79) {\footnotesize $\overline{r}_0$};
\node at (0.22,0.28) {\footnotesize $\overline{r}_f$};

\end{scope}

\end{tikzpicture}
\caption{Example problem with $m^{\mathrm{A}}=10$ UAV task locations.}
\label{fig: an_example}
\end{figure}
